Edge-disjoint paths in expanders: online with removals

We consider the problem of finding edge-disjoint paths between given pairs of vertices in a sufficiently strong $d$-regular expander graph $G$ with $n$ vertices. In particular, we describe a deterministic, polynomial time algorithm which maintains an initially empty collection of edge-disjoint paths $\mathcal P$ in $G$ and fulfills any series of two types of requests: 1. Given two vertices $a$ and $b$ such that each appears as an endpoint in $O(d)$ paths in $\mathcal P$ and, additionally, $|\mathcal P| = O(n d / \log n)$, the algorithm finds a path of length at most $\log n$ connecting $a$ and $b$ which is edge-disjoint from all other paths in $\mathcal P$, and adds it to $\mathcal P$. 2. Remove a given path $P \in \mathcal{P}$ from $\mathcal{P}$. Importantly, each request is processed before seeing the next one. The upper bound on the length of found paths and the constraints are the best possible up to a constant factor. This establishes the first online algorithm for finding edge-disjoint paths in expanders which also allows removals, significantly strengthening a long list of previous results on the topic.

==> Preliminaries.tex <==
\section{Preliminaries}

In this section we present a few simple auxiliary results which we will need in our proofs. 
Let us first give some notation which we will use throughout the paper. Let $D$ be a directed graph, and let $S_1,S_2$ be subsets of its vertices. By $\textrm{Out}_D(S_1,S_2)$ we will denote the set of edges going from $S_1$ to $S_2$, and we denote $\dout_D(S_1,S_2)=|\textrm{Out}_D(S_1,S_2)|$. We similarly define $\textrm{In}_D(S_1,S_2)$ and its cardinality $\din_D(S_1,S_2)$. We also write $\dout_D(v)$ and $\din_D(v)$ for the out- and in- degree of $v$. A digraph is $d$-regular if it both the out- and in-degree of every vertex is $d$. We also denote $e_D(S_1,S_2)=\dout_D(S_1,S_2)+\din_D(S_1,S_2)$, and by $e_D(S_1)$ the number of edges spanned by $S_1$.
%We denote by $\delta^0(D)$ the minimum semidegree of $D$, i.e. the minimum among all in and out-degrees of every vertex.

\ND{other notation here}


\begin{lem}\label{lem:directed factor}
    Given $d \in \mathbb{N}$ and $d_1, d_2 \ge 1$, the edges of a $d$-regular digraph $D$ can be decomposed into $D_1 \cup D_2 \cup \ldots \cup D_d$, where each $D_i$ is a spanning $1$-regular digraph. Moreover, they can all be computed in $O(nd^2)$ time.
\end{lem}
\begin{proof}
We construct an auxiliary bipartite graph $B=(V_1\cup V_2, E)$ where each $V_i$ is a distinct copy of $V(D)$, and $u \in V_1$ and $w \in V_2$ are connected by an edge in $B$ if $(u,w) \in D$. Note that $B$ is $d$-regular, hence it contains a perfect matching which can be found in time $O(n d)$ (see \cite{cole2001edge}). Furthermore, note that such a perfect matching corresponds to a $1$-regular subgraph $D' \subseteq D$. Removing $D'$ from $D$ and repeating the procedure gives the required  decomposition.
\end{proof}

\RN{Mozda dodati expander mixing lemmu ovde, i sta nam ona kaze o broju grana u malim podskupovima.}
\ND{Nisam siguran, ne koristimo je zapravo nigde osim na kraju, gde ionako ne dajemo nikakav ozbiljan dokaz, tako da mozda ne treba trositi reci?}

%  We start with a lemma which shows that in a $d$-regular graph, we can assign to each vertex a set of $d/10$ of its adjacent edges, such that those sets are mutually disjoint.
 

% \begin{lem}\label{lem:assign edges}
%  Let $G$ be a $n$-vertex $d$-regular graph. For each vertex $v$ in $G$ there exists a set $L_v \subseteq E(G)$ of $d/10$ edges incident to $v$, such that $L_v \cap L_w = \emptyset$ for $v \neq w$, and for each $v$ there are at most $1 + d/10$ edges in $\bigcup_{w, w\neq v} L_w$ which are incident to $v$. Furthermore, such an assignment can be found in $O(nd^2)$ time.
% \end{lem}
% \begin{proof}
% If $d$ is even, then by Petersen's theorem $G$ has a $2$-factor, and moreover it can be found in $O(dn)$ time \cite{cole2001edge}. For each cycle in the $2$-factor, assign to each of its vertices precisely one incident edge from the cycle. By removing the $2$-factor, the graph stays even, so we can repeat this $d/10$ times.

% If $d$ is odd, then by the Handshake-lemma, $G$ has an even number of vertices, so we can add a spanning matching $M$ on top of $G$ to get a $(d+1)$-regular multigraph. Again, by Petersen's theorem, it contains a $2$-factor and we can analogously to the previous case get an assignment of $1 + d/10$ edges $L_v$ to each vertex. By removing at most one edge from each $L_v$ which is in $M$, or an arbitrary edge if such does not exist, we get the required assignment.
% \end{proof}

% % An analogous statement holds for directed graphs.
% % \begin{lem}
% %     Let $D$ be a $n$-vertex $d$-regular digraph. For each vertex $v$ in $G$ there exist sets $L^-, L^+_v \subseteq E(D)$, both of size $d/10$, such that:
% %     \begin{itemize}
% %         \item  $L_v^+$ are edges going out of $v$, and $L_v^-$ are going towards $v$.
% %         \item  Further, all sets $L_v^+, L_v^-$ are pairwise disjoint.
% %         \item For each vertex $v\in D$ there are at most $d/10$ edges in $\bigcup_{w} L^+_w$ which contain $v$ as a sink. Analogously, there are at most $d/10$ edges in $\bigcup_{w} L^-_w$ which contain $v$ as a source.
        
% %     \end{itemize}
% %         Furthermore, such an assignment can be found in $O(nd^2)$ time. 
% % \end{lem}
% % \begin{proof}
% % By Lemma~\ref{lem:directed factor}, one can find $d$ directed $2$-factors in $D$. Now, for $d/10$ of those $2$-factors, assign for each vertex $v\in D$ the out-going edge to the set $L_v^+$. Analogously, for another $d/10$ of those $2$-factors, assign for each vertex $v\in D$ the in-going edge to the set $L_v^-$. Note that this assignment satisfies all the requirements, which completes the proof. 
% % \end{proof}

% The next result states that sets of certain size in directed $d$-regular $\beta$-expanders. have good vertex expansion.

% \begin{lem}
% Let $D$ be a $\beta$-expanding $d$-regular $n$-vertex digraph, and let $S$ be a set of its vertices, and let $R$ be a subset of its edges with $|R|\leq \frac{nd}{10^9}$. Then we the following holds
% $$
%     |N_{D-R}^\star(S)|\ge \begin{cases}
%         \min\{n/2-|S|,|S|/20\} & \text{if $\beta n\leq |S| \le  n/2$} \\
%         \min\{\beta n-|S|,2|S|\}  & \text{if $< |S| \le \beta n$.}
%     \end{cases}
% $$
% \end{lem}
% \begin{proof}
% Suppose for contradiction that the first inequality does not hold. Then, since $|R|<\beta nd/11\leq |W|d/100$ we have
% $$
%     |E_D[S\cup N_{D-R}(W)]|\geq (\frac{9d}{10}-1)|W|-2|R|\geq  %\frac{4d}{5}|W|-\frac{3d}{40}|W|\geq 
%     \left(|W|+\frac{|W|}{20}\right)\frac{2d}{3}\geq |W\cup N_{G''}(W)|\frac{2d}{3},
% $$
% \end{proof}

% \begin{lem}\label{cl:connection} 
% Let $D$ be a directed $d$-regular $\beta$-expander and let $D'\subseteq D$ such that $\delta^0(D')\geq \frac{4}{5}d$, and with $\beta=1/750$. Then for every $R \subseteq E(D')$ with $|R| \le nd / 10^9$, and every two disjoint subsets $A, B \subseteq V(G)$ of sizes $|A|, |B| \ge n / 10^8$, there exists a path between $A$ and $B$ of length at most $320$ contained in the subgraph $D''=(V(D'),E(D') \setminus R)$. Moreover, the path can be found in time $O(n)$.
% \end{lem}

% \begin{proof}
% For every subset of edges $R \subseteq E(D')$, $|R| \le nd / 10^9$, each set of vertices $S \subseteq V(D)$ of size $\beta n \le |S| \le n/2$ satisfies 
% $$
%     |N^\star_{D''}(S)|> \min\{n/2-|S|,|S|/20\}.
% $$
% Indeed, if that was not the case, then since $|R|< |S|d/100$ we have
% $$
%     |E_D[S\cup N_{D''}^\star (S)]|\geq \frac{4d}{5}|S|-2|R|\geq  %\frac{4d}{5}|S|-\frac{3d}{40}|S|\geq 
%     \left(|S|+\frac{|S|}{20}\right)\frac{2d}{3}\geq |S\cup N_{D''}(S)|\frac{2d}{3},
% $$
% which contradicts the assumption that $D$ is a $\beta$-expander. Further, note that for every set $S$ with $n/10^8\leq |S|<\beta n$ we have $|N_{D''}(S)|\geq \min\{2|S|,\beta n-|S|\}$. Indeed, otherwise we have 

% $$
%     |E_D[S\cup N_{D''}^\star (S)]|\geq \frac{4d}{5}|S|-|R|\geq  %\frac{4d}{5}|S|-\frac{3d}{40}|S|\geq 
%     3|S|\frac{d}{6}\geq |S\cup N_{D''}^\star (S)|\frac{d}{6},
% $$
% a contradiction with the first property of a $\beta$-expander. This in turn implies that $A$ can reach a set of size $\beta n$ by a directed path of length at most $20$ (as $2^{20}|A|\geq \beta n)$. Similarly, there is a set of vertices of size $\beta n$ which can reach $B$ by a directed path of length at most $20$.

%  Finally, by using the property from the beginning of the proof, there is a path of length at most $300$ between those two balls, as 150 steps are enough to reach $n/2$ vertices from a set of size $n/750$ (since $\frac{1}{750}(1+1/20)^{150}\geq \frac{1}{2}$), giving the desired path of length at most $320$.

% Since finding the first neighbourhood of a set of vertices takes only $O(n)$ time, and we have to do it a constant number of times, the required path can be found in $O(n)$ time.
% \end{proof}


\begin{defn}[Alternating walk]
    \label{def:alternating}
    Given a digraph $D$ and subsets of edges $E_1, E_2 \subseteq E(D)$, we say that a sequence of vertices $(v_1, v_2, \ldots, v_k)$, which are not necessarily distinct, forms an \emph{$(E_1, E_2)$-alternating walk} $W$ from $v_1$ to $v_k$ if $(v_{2i+1}, v_{2i+2}) \in E_1$ for every $0 \le i \leq  k/2 - 1$, and $(v_{2i+1}, v_{2i}) \in E_2$ for every $1 \le i < k/2$.

    \noindent
    \textbf{Note:} the direction of the edges along $W$ does not form a directed walk. In particular, they form an anti-directed walk.
\end{defn}

==> main_theorem.tex <==

\section{Disjoint paths via Edge-Oracle}

% The proof of Theorem \ref{thm:main} hinges on the following auxiliary game. Given a digraph $D$ and $m, d \in \mathbb{N}$, we define the \emph{$(m,d)$-Edge game} on $D$ between two players, \emph{Client} and \emph{Oracle}, as follows. At the beginning of the game set $H = (V(D), \emptyset)$, that is, $H \subseteq D$ is a spanning subgraph of $D$ with no edges. In each step of the game, Client has two types of requests:
% \begin{itemize}
%     \item \texttt{add-out-edge $v$}: Given a vertex $v \in V(D)$ with $\deg^+_H(v) < d$, Oracle selects an edge $e = (v, w) \in D \setminus H$ such that $\deg^-_H(w) < \lfloor d/4 \rfloor$, returns it to Client and updates $H := H \cup e$. If such an edge does not exist, Oracle loses the game. \textbf{Note:} This request is only allowed if $e(H) < m$. 
%     \item \texttt{remove-edge $e$}: Remove a given edge $e \in H$ from $H$.
% \end{itemize}
% Each request has to be fulfilled before seeing the next one. We say that Oracle wins a game if they can satisfy any infinite series of requests.

% % Our key lemma shows that Oracle has a winning strategy if $B$ is a sufficiently strong expander. We postpone the proof of it for the next section. 

% \begin{restatable}{lem}{oracle}\label{lem:oracle}
% Let $D$ be a $d$-out-regular digraph with $n$ vertices, for some $d \ge 10$. Suppose that for every set $S \subset V(D)$ of size $|S| \leq \beta n$ we have $e_B(S) \leq K \beta |S|d$, for some $\beta < 1/500$ and $K > 0$. Then Oracle has a strategy to win the $(\beta nd / K, \lfloor d/2 \rfloor)$-Edge game on $D$. Moreover, Oracle can respond to each request in $O(n^2 d)$ time.
% \end{restatable}

% We postpone the proof for the next section. In the remainder of this section, we show how to apply the above lemma to prove Theorem~\ref{thm:main}. 

% % Before we give the proof, we will need the following standard result.

% We are now ready to prove our main result.
\begin{proof} [ of Theorem~\ref{thm:main}]
Let $r=\frac{nd}{10^8\log_4n}$. For each vertex $v\in V(G)$, let $L^+_v$ be the subset of out-edges adjacent to $v$ given by \Cref{lem:assign edges}, and $L_v^-$ its in-edges. Denote by $G^+$ the graph formed by all $L_v^+$, and define $G^-$ analogously. Denote by $G'=G-(G^-\cup G^+)$ the remaining edges.


 By Lemma~\ref{cl:connection}, one can find very short paths (of length 320) in $G'$ between two large subsets of size at most $n/10^8$, and this will be the main role of the subgraph $G'$ in the rest of the proof.

Now that we set up $G'$, we use the remainder of the graph to construct the requested paths. More precisely, the requested paths will almost exclusively use those remaining edges, and a few edges from $G'$ to complete the path. The key tool to do this will be Lemma~\ref{lem:oracle}; let us briefly outline the remainder of the proof. Suppose we have dealt with some requests of the adversary, and at a given point the adversary requests a pair $(a,b)$. We want to construct two large trees of logarithmic depth rooted at $a$ and $b$ respectively, which use the free edges in and are contained in $G^+$ and $G^-$, respectively. The tree rooted at $a$ will have all edges oriented towards the leaves, while the other tree will have edges oriented towards the root $b$. Since the trees will be of size larger than $n/10^8$, we will use the claim above to complete the path, and subsequently we will remove all the edges in the trees which are not used in the path. 
The crucial ingredient which will allow us to repeat this procedure indefinitely is Lemma~\ref{lem:oracle}. 
% In particular, for the graph $G^+$ we will define an auxilliary bipartite graph whose two color classes $A,B$ will be two copies of $V(G)$, with an edge between every pair which corresponds to an edge in some $L_v^+$. Starting at vertex $a\in A$, we can find a star of size $\varepsilon d$, whose leaf $S$ set is in $B$, then we look at the vertices in $A$ which correspond to $S$ (as $S\subseteq V(G)$), and again find a star for each of those vertices. The union $S'$ of the leaves of those stars in $B$ will be of size at least, say, $5|S|$, because our graph is a $\beta$-expander. So we can look at the vertices of $A$ which correspond to $S'\setminus S$, and continue this procedure until the vertex set which we obtain is of size at least $n/10^8$. This will clearly correspond to a large tree in $G^+$. We can perform the same procedure for the vertex $b$ in the graph $G^-$. Now, by Claim~\ref{cl:connection}, there is a short path between those trees, which in the end gives a path between $a$ and $b$. By the properties of the Oracle, we can remove all edges which are not used in the path, and still be able to continue the procedure, as long as the number of currently used paths does not exceed $\varepsilon nd $. For this, it is crucial that in the auxiliary bipartite graph we always have that every vertex in $B$ is not used many times, which on the other hand guarantees that in $G^\star$ each vertex is not touched too many times by the established paths.
The details are given below.



We construct bipartite graph $B^+=(V_1\cup V_2, E^+)$ where each $V_i$ is a distinct copy of $V(G)$ and $(v,u) \in E^+$ iff $(v,u) \in L_v$. Define $B^-$ analogously. Note that $B^+$ and $B^-$ are one-sided $d'$-regular, for $d'=d/10$. We, putting ourselves in the role of Router here, access the edges of $B^+$ (and, consequently, the corresponding edges in $G$) through the Client--Oracle $m$-Edge game, for $m = \frac{nd'}{10^7}$, as Client. In particular, we invoke \Cref{lem:oracle} applied to the graph $B^+$ (with $d/10$ instead of $d$); we can indeed do this, as for any set $S\subseteq V(B^+)$ of size $|S|\leq \beta n$ it holds that $e_{B^+}(S)\leq \beta d|S|\leq 10\beta d'|S|$. The same holds for $B^-$.
%Indeed, if $S=S_1\cup S_2$ is such that $S_1\subseteq V_1$ and $S_2\subseteq V_2$ 
Now we are ready to describe the algorithm.

We maintain a subset $H\subset {B^+}$ of auxiliary edges in ${B^+}$. Using the oracle guaranteed by Lemma~\ref{lem:oracle}, we will utilize $H$ to find large trees of small depth $G^+$. After doing the same with $B^-$ and $G^-$, we use the edges of $G'$ to complete the path between a requested pair of vertices by connecting the two large trees.

Let us now describe the procedure for $B=B^\star$.

Initially we set $H=\emptyset$. 
We make sure that the following invariants hold:
\begin{enumerate}
    \item\label{p:adding to H} We only add edges to $H$ using the oracle, so as long as a vertex in $V_1$ has degree less than $d_1:=d'/3$ in $H$, we can add another edge to it using the oracle, so that $d_H(y)\leq d_2:=d'/10$ at every point.
    \item\label{p:degrees} Before the next request is made, we have that $d_H(x)\leq 2d_1/3$ for all $x\in V_1$. Furthermore, after a request is satisfied, every edge in $H$ corresponds to an edge in $G-G'$ used in some path which we constructed to satisfy a request.
    \item\label{p:edges in F} For each pair in $\mathcal{P}$ we used at most $320$ edges in $G-G'$ for making the connection.
\end{enumerate}
In what follows, for a set $S\subseteq V(G)$ we denote by $S^A$ the set of vertices in $A$ which correspond to vertices in $S$ (recall that $A$ is a copy of $V(G)$).
Suppose the adversary requests the vertex pair $(a,b)$ in $G$. We do the following procedure. 

Since $d_H(a)\leq 2d_1/3$, we can use the Oracle to add $d_1/3$ edges adjacent to $a$ in ${B}$ to the graph $H$.
Let $X$ be the set of those $d_1/3$ vertices. Let $R=\{a\}$, and do the following until $|{X^A}\cup R|\geq n/10^8$, always maintaining the invariant $|X|\geq 4|R|$.
For all vertices in $X^A-R$ add $d_1/3$ adjacent edges to $H$, using the oracle. Since the number of those edges is $(|X|-|R|)d_1/3\geq \frac{1}{4}|X|d_1=\frac{1}{12}|X|d'$, the set of vertices $X'$ in $V_2$ which are adjacent to at least one of them is of size at least $|X'|\geq 5|X|$, otherwise a set of size at most $6|X|$ spans more than $10\beta d'|X|$ edges in ${B}$. Let $R:=R\cup X^A$, and let $X:=X'$, so that $|X|\geq 4|R|$ again.

Note that each time we can successfully add $d_1/3$ edges to each vertex in $ X^A-R$ using the oracle, because $R$ is precisely the set of vertices to which we already added the $d_1/3$ edges, and all remaining vertices by assumption had at most $2d_1/3$ neighbours in $H$ before starting the procedure.
 
Now, let $W^\star= X^A\cup R$ be the set obtained at the end of this procedure. 
Note that every vertex $w\in W^+$ (viewed as a subset of vertices in the graph $G^+$) is such that there exists a directed path of length at most $\log_5n$ from $a$ to $w$ using only edges corresponding to the edges added to $H$ in the above procedure. Analogously, there is a directed path between every $w\in W^-$ and $b$ of length at most $\log_5n$.


% . If one of the vertices in $W$ is $b$, then we can stop. Otherwise, look at the copy of $b$ in $V_1$, and repeat the same procedure as for $a$, or stop as soon as the set $X$ from the procedure contains any vertex in $W$. Note that we can always use the oracle to add new edges, since $X$ is always disjoint from $W$, so we never request vertices in $W^A$ again to add new edges to $H$. Let $U=X^A\cup R$ be the set obtained in the end of the procedure we did for vertex $b$.  

If $W^-$ and $W^+$ do not already intersect, we have two disjoint sets of vertices of size at least $n/10^8$ in $G$. For each individual previous request we used only $320$ edges in $G'$, hence all but $320r\leq \frac{nd}{10^8}$ edges in $G'$ are free. By \Cref{cl:connection} there exists a directed path between $W^-$ and $W^+$ of length at most $320.$ This gives the required path in $G$ between $a$ and $b$ of length at most $2\log_4n+320= O(\log n)$.

What is left to do, is to remove the unused edges in $H^+$ and $H^-$. Using the oracle, we can request the removal of all edges which do not correspond to the part of the found path between $(a,b)$ in $G^+$ and $G^-$, respectively. Note that after this removal process, Property (\ref{p:degrees}) is still satisfied. Indeed, by construction, every vertex in $V_2$ has at most $d_2$ neighbours in $H.$ Further, notice that a vertex $v$ in $V_1$ has only two types of adjacent edges in $H$. First, the initial edges of the paths when $v$ is in a requested pair; the number of those is by assumption at most $d_1/3$. On the other hand, we have the edges $(v,u)$ which succeed an edge $(w,v)$ on some path in the current collection of paths. Hence, when $(v,u)$ is added to $H$, then $(w,v)$ was also added to $H$; since we have at most $d_2=d_1/3$ edges of the form $(w,v)$ (for different $w\in V_1$) added to $H$, we conclude that $v$ has at most $d_1/3$ of the second type. Hence, we conclude $d_H(v)\leq 2d_1/3$ when a new pair is requested.

Now, if the adversary requests a pair $(a,b)$ in $\mathcal P$ to be removed, then, using the oracle, we simply remove all edges in $H^+$ and $H^-$ used for the corresponding path, and we remove all edges in $G'$ used for it. We remove the pair $(a,b)$ from $\mathcal P$, and we free all the edges in $G$ which are used for this path. 

Finally, the number of used edges in $H$ is at any point at most $r(2\log_4n+320)+2\frac{n}{10^8}d_1\leq \frac{nd'}{10^7}$, where the first term is the number of edges used for the paths which connect pairs in the current $\mathcal P$, and the second term bounds the number of edges in $H$ used for the path we are currently building. So we are always able to successfully add a new edge to $H$. 
To complete the proof, note that each time we get a request to add a path, we make $O(nd)$ requests to the Oracle to add edges to $H$, each of which costs $O(n^2d)$ time. Connecting the two large sets of vertices to complete the paths only takes $O(n)$ steps. Hence, the total time needed to satisfy such a request is $O(n^3d^2)+O(n)=O(n^3d^2)$.
On the other hand, when removing a path, one only needs to call the Oracle $O(\log n)$ times, so evidently $O(n^3d^2)$ steps are enough.


\end{proof}

==> oracle.tex <==

\section{Proof of the Oracle Lemma}

We introduce a few definitions in order to keep the proof of Lemma \ref{lem:oracle} concise.

\begin{defn}[Complements] Given a digraph $D$ and a subset $U \subseteq V(D)$, we denote with $\compl{U} = V(D) \setminus U$ the complement of $U$ in $V(D)$. Similarly, given a subset of edges $F \subseteq E(D)$, we denote with $\compl{F} = E(D) \setminus F$ the complement of $F$ with respect to $D$.
\end{defn}

The following definition is inspired by the notion of alternating paths used in matching algorithms.

\begin{defn}[Alternating paths]
    Given a digraph $D$ and subsets of edges $E_1, E_2 \subseteq E(D)$, we say that a directed path $P = (e_1, e_2, \ldots, e_k)$ in $D$ is \emph{$(E_1, E_2)$-alternating} if $e_i \in E_1$ for odd $i$, and $e_i \in E_2$ for even.
\end{defn}

For the convenience of the reader, we restate the Oracle Lemma.

\oracle*

\begin{proof}
We start with a few definitions and describe invariants which are maintained throughout the game. Denote $d_1=\lfloor d/2 \rfloor$, $d_2= \lfloor d_1 / 2 \rfloor > d/5$, and $c = \beta/100$. Given a graph $F$, define $\Sat(F) \subseteq V(D)$, the set of \emph{saturated} vertices, and $\Low(F) \subseteq V(D)$, the set of those with too few neighbours which are not saturated (or, equivalently, too many saturated neighbours), as follows:
$$
    \Sat(F) =\{v \in V(D) \colon \deg^-_F(v) \ge d_2/2 \} \quad \text{ and } \quad \Low(F) =\{v \in V(D) \colon \deg^+_B(v, \Sat(F)) \ge d_1/2\}.
$$
Let us denote with $H_i$ the graph consisting of `active' edges after handling $i$-th Client's request. Moreover, after $i$-th request we (as Oracle) also maintain a carefully chosen (initially empty) set of \emph{buffer} edges $\Buff_i \subseteq \compl{H_i}$, such that the following properties are satisfied for $F_i = H_i \cup \Buff_i$:
\begin{enumerate}[(P1)]
    \item\label{p:Y} for each $v \in V(D)$ we have $\deg^-_{F_i}(v) \le d_2$,
    \item\label{p:X} for each $v \in \Low(F_i)$ we have $\deg^+_{F_i}(v)=d_1$,
    \item\label{p:A} for each $v \in \compl{\Low(F_i)}$ we have $\deg^+_{\Buff_i}(v) = 0$, and
    \item\label{p:size} $|\Low(F_i)| < \lfloor cn \rfloor$.
\end{enumerate}
In the beginning we have $H_0 = \Buff_0 = \emptyset$ thus, as $d_2 \ge 1$, $\Low(F_0) = \Sat(F_0) = \emptyset$ and all the properties are trivially satisfied. 

\paragraph{Adding an edge to $H$.} Suppose \ref{p:Y}--\ref{p:size} hold after $i$-th request, for some $i \ge 0$, and $H_i$ contains less than $cnd$ edges. We now show how to respond to Client's request for an edge incident to some $v \in V(D)$ with $d_{H_i}(v)< d_1$. We distinguish two cases.

\paragraph{Case 1: $v \in \Low(F_i)$.} As $d_{H_i}(v) < d_1$ and $d_{F_i}(v) = d_1$, there exists an edge $e = (v, w) \in \Buff_i$. From $\deg^-_{F_i}(v) \le d_2$ we conclude $\deg_{H_i}(w) < d_2$, thus $e$ satisfies requirements of the game and we return it to Client. Update $H_{i+1} := H_i \cup e$ and $\Buff_{i+1} := \Buff_i \setminus e$. Then $F_i = F_{i+1}$ and, consequently, $\Sat(F_i) = \Sat(F_{i+1})$ and $\Low(F_i) = \Low(F_{i+1})$, thus \ref{p:Y}--\ref{p:size} remain satisfied.

\paragraph{Case 2: $v \notin \Low(F_i)$.} From $\deg_{H_i}(v) < d_1$ we have
$$
\deg_{\compl{H_i}}(v) > d - d_1 \ge d/2 > d_1 / 2,
$$
thus $v \notin \Low(F_i)$ implies there exists an edge $e = (v,w) \in \compl{H_i}$ with $w \notin \Sat(F_i)$. Such $e$ satisfies requirements of the game by \ref{p:Y}, thus we update $H_{i+1} := H_i \cup e$ and return $e$ to Client. If $\deg_{F_i}(w) < d_2 - 1$, then $\Buff_{i+1} := \Buff_i$ suffices. Suppose that this is not the case, that is, $\deg_{F_i}(w) = d_2 - 1$. Finding appropriate set $\Buff_{i+1}$ in this case is the heart of the strategy, and it is done using Algorithm \ref{alg:main}. For the rest of the proof we analyse this algorithm and show its correctness.

\begin{algorithm}[h]
    $\Buff_{i+1} := \Buff_i$, $\Low_{i+1} := \Low(F_i)$, $\Sat_{i+1} = \Sat(F_i) \cup \{w\}$, $F' := F_i \cup \{(v,w)\}$

    \While{there exists $x \in \compl{\Low_{i+1}}$ such that $\deg^+_B(x, \Sat_{i+1}) \ge d_1 / 2$}{
        \While{$\deg_{F'}(x) < d_1$}{
            Find an $(B \setminus F', \Buff_{i+1})$-alternating path $P$ from $x$ to some $y \in V(D)$ with $\deg^-_{F'}(y) < d_2$
            
            \For{$e \in P$}{
                \textbf{if} $e \in \Buff_{i+1}$ \textbf{then} remove $e$ from $\Buff_{i+1}$ and $F'$

                \textbf{else} add $e$ to $\Buff_{i+1}$ and $F'$
            }

            \textbf{if} $\deg^-_{F'}(y) \ge d_2/2$ \textbf{then} add $y$ to $\Sat_{i+1}$
        }
        Add $x$ to $\Low_{i+1}$
    }
  \caption{Building $\Buff_{i+1}$.}
  \label{alg:main}
\end{algorithm}

Let us, for now, assume that line 5 is well-defined, that is, whenever it is executed it finds a desired path. Note that throughout the algorithm we maintain: 
\begin{enumerate}[(i)]
    \item $\deg_{F'}(y) \ge d_2/2$ for $y \in \Sat_{i+1}$, $\deg_{F'}(y) \le d_2$ for $y \in V_2$,
    \item $\deg_{F'}(x) = d_1$ for $x \in \Low_{i+1}$, $\deg_{\Buff_{i+1}}(x) = 0$ for $x \in \compl{\Low_{i+1}}$, and
    \item $\deg_{B}(x, \Sat_{i+1}) \ge d_1 / 2$ for $x \in \Low_{i+1}$.
\end{enumerate}
The following facts are also easy to check:
\begin{itemize}
    \item After each iteration of the \textbf{while} loop in line 3 one vertex gets added to $\Low_{i+1}$.
    \item After the \textbf{for} loop (line 5) finishes, $\deg_{F'}(x)$ and $\deg_{F'}(y)$ increase by $1$, whereas $\deg_{F'}(v)$ remains the same for every intermediate vertex in $P$. In particular, with each iteration of the \textbf{while} loop in line 4, $\deg_{F'}(x)$ increases by $1$. Therefore, the loop repeats at most $d_1$ times. 
    \item The previous two observations (and the assumption about line 10) imply that the algorithm eventually terminates. Moreover, once it terminates we have $Y(F_{i+1}) = Y(F_i) \cup Y'$ and $X(F_{i+1}) = X(F_i) \cup X'$, for $F_{i+1} = H_{i+1} \cup A_{i+1}$.    
\end{itemize}
Properties \ref{p:Y}--\ref{p:A} follow easily from the description of the algorithm and these facts. It remains to show that \ref{p:size} always holds and that, whenever line 4 is executed, a desired path $P$ exists. In both cases we use the following inequality, which holds throughout the execution of the algorithm:
\begin{equation} \label{eq:size_eq}
    d_2 |\Sat_{i+1}| \le cnd + |\Low_{i+1}|d_1.
\end{equation}
The left hand side is equal to $e_{F'}(V_1, \Sat_{i+1})$ (by \ref{fact:deg}), and the right hand side upper bounds $e(F')$.

\begin{claim*}
\ref{p:size} holds.
\end{claim*}
\begin{proof}[ of Claim]
Suppose, towards a contradiction, that at some point during the execution of the algorithm we have $|\Low_{i+1}| = \lfloor cn \rfloor$. Let us pause the execution at that point and analyse the current situation.

From \eqref{eq:size_eq} and $|\Low_{i+1}| \le c n$ we conclude $|\Sat_{i+1}| \le 8 cn$, with room to spare. As $S = \Low_{i+1} \cup \Sat_{i+1}$ is of size $|S| \le 9 cn < \beta n$, by the assumption of the lemma we have
\begin{equation} \label{eq:contra}
    e_B(\Low_{i+1}, \Sat_{i+1}) \le 10 \beta |S| d < 100 |\Low_{i+1}| \beta d.
\end{equation}
Utilising \ref{fact:deg}, we have
$$
    e_B(\Low_{i+1}, \Sat_{i+1}) \ge |\Low_{i+1}| d_1 / 2 > |\Low_{i+1}| d / 5,
$$
thus get a contradiction with \eqref{eq:contra} follows from $\beta < 1/500$.
\end{proof}

\begin{claim*}
    Whenever line 4 is executed, a desired path exists.
\end{claim*}
\begin{proof}[ of Claim]
    As in the proof of the previous claim, suppose, towards a contradiction, that at some point during the execution of the algorithm we reach line $4$ and a desired path does not exist. Pause the execution at that point.
    
    Let $\Delta = \Buff_{i+1} \setminus \Buff_i$, and note that the edges in $\Delta$ do not touch vertices in $\Low_i$. Let $Y \subseteq V_2$ denote the endpoints of all $(B \setminus F', \Buff_{i+1})$-alternating paths. For every $y \in Y$ we necessarily have $\deg_{F'}(y) = d_2$, as otherwise a desired path exists. Let us consider $Y' = Y \setminus \Sat_i$. As $x \notin \Low_i$, we have $Y' \neq \emptyset$. Furthermore, as $y \notin \Sat_i$, $\deg_{F'}(y) = d_2$, and all the newly added edges are contained in $\Delta$, we have $\deg_{\Delta}(y) \ge d_2/2$. Let $X' = N_{\Delta}(Y')$, and note that $X' \subseteq \Low_{i+1} \setminus \Low_i$. For each $x \in X'$ we have
    $$
        \deg_{B \setminus F'}(x, \compl{\Sat_i}) \ge d - d_1 - d_1/2 > d/4
    $$
    and $N_{B \setminus F'}(x, \compl{\Sat_i}) \subseteq Y'$, as otherwise we get a vertex $v \notin Y$ which is also an endpoint of a $(B \setminus F', \Buff_{i+1})$-alternating path from $x$. We have already established $|X'| \ge |Y'|$ and $|X'| \le |\Low_{i+1}| < cn$ (this was done in the previous claim), thus by the assumption of the lemma we have
    $$
        |X'| d / 4 \le e_{B \setminus F'}(X', Y') \le e_{B}(X', Y') < 2|X'| \beta d,
    $$
    which is a contradiction for $\beta < ?$. Therefore, a desired path must exist.
\end{proof}

\paragraph{Removing an edge from $H$.} Suppose Client requests an edge $e = (v,w)$ to be removed from $H_i$, that is, $H_{i+1} := H_i \setminus e$. Set, tentatively, $\Buff_{i+1} := \Buff_i$. If $v \in \Low(F_i)$, then the properties are satisfied and we can continue to the next request. Otherwise, if $v \notin \Low(F_i)$, we need to further clean-up $\Buff_{i+1}$ by repeating the following: $x \in \compl{\Low(F_{i+1})}$ remove all the edges incident to $x$ in $\Buff_{i+1}$, where $F_{i+1} = H_{i+1} \cup \Buff_{i+1}$. If no edge is removed from $\Buff_{i+1}$ in some iteration, terminate the updating process. A couple of simple observations: (a) no edge is added to $\Buff_{i+1}$ nor $H_{i+1}$ during this process, thus $F'$, and consequently $\Sat(F_{i+1})$ and $\Low(F_{i+1})$, can only shrink throughout the process; (b) we only remove edges in $\Buff_{i+1}$ incident to vertices which are not in $\Low(F_{i+1})$. One easily checks now that all the properties are satisfied.
\end{proof}

% \RN{Nemanjin ispis dokaza ispod.}

% \begin{proof}
% Denote $d_1=d/3$ and $d_2=d/10$. Throughout the game we maintain a set of edges $A \subseteq B \setminus H$ and subsets $X \subseteq V_1$ and $Y \subseteq V_2$ such that the following holds:
% % We (having the role of Oracle) start by initializing a few auxiliary sets which will change throughout the game. 
% % Let $R \subseteq E$ be set of edges which are used to satisfy the requests. Before the game starts, we have $R=\emptyset$. Further, define the graph $A$ to be a graph of auxiliary edges, which we also set to $A := \emptyset$ in the beginning. Throughout the game we also maintain two sets of vertices, $X \subseteq V_1$ and $Y \subseteq V_2$ (both initially empty), such that the following invariants hold:
% \begin{enumerate}
%     \item\label{p:Y} $Y=\{y\in V_2: d_H(y)\geq d_1/10\}$ where $H=H_0\cup H_1$.
%     \item\label{p:X} $X=\{x\in V_1: |N_B(x)\cap Y|\geq d_1/2\}$ and for each $x\in X$ we have $d_H(x)=d_1$.
%     \item\label{p:size} $|X|\leq n/10^5$.
% \end{enumerate}

% Each edge in $B-H$ we call a \emph{free} edge, and if $(u,v)$ is free, then we say that $v$ is a free neighbour of $u$.
% Clearly, in the beginning all the invariants are satisfied. Suppose that $H_0$ currently contains less than $m$ edges, and suppose the adversary requests some vertex $v\in V_1$ with $d_{H_0}(v)<d_1$. 

% If $v\in X$, then at least one of its $d_1$ edges to $N_H(v,V_2)$ is not in $H_0$, so we move this edge from $H_1$ to $H_0$. Note that all invariants are still satisfied, so in this case we successfully completed the adversary's request.


% If $v\notin X$, we do the following procedure. 

% Since $N_B(v,Y)< d_1/2$, there is at least one edge $(v,u)$ in $B-H_0$ with $u\notin Y$, because $N_{B-H_0}(v,V_2)\geq d-d_1>d_1/2$, so we add $(v,u)$ to $H_0$. 
% % Since we added an edge to $H=H_0\cup H_1$, then possibly the vertex $u$ now has $d_1/10$ edges in $H$.
% If $d_H(u)<d_1/10$ after adding the edge $(v,u)$ to $H$, then all the invariants are still satisfied, so we fulfilled the adversary's request successfully.

% Otherwise, we add the vertex $u$ to $Y$ and observe that by doing this, there might be vertices $t\notin X$ such that $|N_B(t,Y)|\geq d_1/2$, so let $T$ be the set of such vertices, which we have to add to $X$, and order them arbitrarily. Let $X_0:=X$ and $Y_0:=Y$.

% Now we do the following. One by one, for each vertex $t\in T$, we try to add $d_1-d_H(t)$ of its free edges to $H_1$, in order to maintain Property~\ref{p:X}. More precisely, for each $t$ we will try to find $d_1-d_H(t)$ vertices $u\in N_{B-H}(t,V_2-Y_0)$, such that $d_H(u)< d_2$. If we succeed in doing this for vertex $t\in T$, we add it to $X$. Each time we add a new auxiliary edge to a vertex $t\in T$, we again look at all vertices $u$ which now have at least $d_1/10$ edges in $H$, and we add them to $Y$.
% As before, we add to $T$ the set of vertices which are supposed to be added to $X$, i.e. the set of $t\notin X$ such that $|N_B(t,Y)|\geq d_1$. When a vertex $t$ is added to $X$, we remove it from $T$ and do the same procedure for the next vertex in $T$.

% If at some point there is a vertex $t\in T$ for which there is no vertex $u\in N_{B-H}(t,V_2-Y_0)$ such that $d_H(u)< d_2$, we know that at least $d-d_1-d_1/2$ free neighbours of $t$ are in $Y_{bad}:=\{u\in Y-Y_0: d_H(u)= d_2\}$. Indeed, $t$ has $d$ neighbours in $B$, out of which at most $d_1$ of then form edges in $H$, and at most $d_1/2$ are in $Y_0$ since $t\notin X_0$.
% Before we continue with adding another edge adjacent to $t$ to the graph $H_1$, we prove the following claim.

% \begin{claim*}
% It always holds that $|X|< n/10^5$,
% %with $c\ll\varepsilon\alpha$.
% \end{claim*}

% \begin{proof}
% Suppose the contrary, that at some point $|X|\geq n/10^5$. Since we are adding vertices to $X$ one by one, observe the first point when $|X|= n/10^5$. Observe that by our algorithm, at every point $Y$ indeed contains all the vertices as described in the first invariant, while there might be some vertices in the current $T$ which need to be added to $X$ to satisfy the second invariant, but this will have no effect on the argument.

% Let us first show that $|Y|\leq 20|X|$.
% Let us estimate $e_H(V_1,Y)$ in two ways. More precisely, we show that 
% \[
% c nd+|X|d_1\geq e_H(V_1,Y)\geq |Y|\frac{d_1}{10}.
% \]
% For the first inequality, observe that the LHS is a bound on the total number of edges in $H$, as the first term bounds the number of edges in $H_0$, and all other edges in $H$ come from the at most $d_1$ neighbours of each vertex in $X$. For the second inequality observe that by the first invariant, each vertex in $Y$ has at least $d_1/10$ adjacent edges in $H$. By plugging in the values of $c=1/10^7$ and $d_1=d/3$, and recalling that $|X|=n/10^5$, this implies that $|Y|\leq 11 |X|$.

% In order to get a contradiction, we estimate $e_B(X,Y)$ in two ways. More precisely, we show
% \[
%     |X|\frac{d_1}{2}\leq e_B(X,Y)\leq 120|X|\beta d.
% \]
% Indeed, the first inequality holds by the second invariant (every vertex that is added to $X$ must satisfy this condition, even though there might be other vertices $x$ outside of $X$ at the moment for which we also have $N_B(x,Y)\geq d_1/2$).  The second inequality holds since by assumption the set $S=X\cup Y$, which is of size at most $12|X|=12 n/10^5 \leq \beta n$, can contain at most $10|S|\beta d$ edges in $B$. 
% Since $d_1=d/3$, the inequality above gives a contradiction and finishes the proof of the claim.
% \end{proof}

% \noindent\textbf{Adding auxiliary edges to $t$}.
% Now we perform the following procedure. Look at the set $S_1$ of the at least $d-d_1-d_1/2$ free neighbours of $t$ in $Y_{bad}$. Note that 
% %in $H_1$ each vertex in $S_1$ has degree at least $d_2-d_1/10$  
% $d_{H_1}(y,X-X_0)\geq d_2-d_1/10$ for every vertex $y\in Y_{bad}$, since every such vertex has $d_2$ adjacent edges in $H$, and since $y\notin Y_0$, all but at most $d_1/10$ of those edges have vertices in $N_{H_1}(y,X-X_0)$. Observe the neighbourhood $S_1'$ of $S_1$ in the graph $H_1[S_1,X-X_0]$, and note that $S_1'$ is of size at least $5|S_1|$ because of local density (otherwise a set of size at most $6|S_1|$ spans at least $|S_1|(d_2-d_1/10)=|S_1|d/15> |S_1|\beta d$ edges). Now, since $S_1'\subseteq X-X_0$, if we find a free neighbour $y$ outside of $Y_{bad}\cup Y_0$ of any vertex in $x\in S_1'$, then we can add that edge $(x,y)$ to $H_1$, and remove one of the edges $(x,y')$ (where $y'\in S_1$) from $H_1$. Now add edge $(t,y')$ to $H_1$. 

% In the other case, if there is no free neighbour of $S_1'$ outside of $Y_{bad}\cup Y_0$, look at the set $S_2$ of free neighbours of $S_1'$ which are not in $Y_0$ (hence are in $Y_{bad}$). Since the number of free edges touching a single vertex in $S_1'$ and which go to $S_2$ is at least $d-d_1-d_1/2$, because of local density again we have that $|S_2|\geq 5|S_1'|$. As before, in $H_1$ each vertex $y\in S_2\subseteq Y_{bad}$ has degree $d_{H_1}(y,X-X_0)\geq d_2-d_1/10$ . Observe the neighbourhood $S_2'\subseteq X-X_0$ of $S_2$ in the graph $H_1$, and note that $S_2'$ is of size at least $5|S_2|$ because of local density. 

% We continue the process, checking if there is a vertex $x\in S_i'$ with a free neighbour $y$ outside $Y_0\cup Y_{bad}$. 
% If there is no such vertex $x$, we again obtain the set $S_{i+1}$ of free neighbours of $S_i'$ which are in $Y_{bad}$ of size precisely $5|S_i'|$, and subsequently a set $S_{i+1}'\subseteq X-X_0$ (of neighbours of $S_{i+1}$ in the graph $H_1$) of size precisely $5|S_{i+1}|$.
% Since $S_i'\subseteq X$ and $|X|\leq  n/10^5$, at some point we find the described vertex $x$. Indeed, $S_{i+1}'$ is always by a factor of $25$ larger than $S_i'$, so at some point $S_i'$ will be too large to be contained in $X$.

% Now, observe the (directed) walk which connects $t$ and $x$ and which goes through $S_1,S_1',S_2,S_2',\ldots S_i,S_i'$, and consider a (directed) path $P$ contained in it which connects $t$ and $x$. Add every free edge in $P$ to $H_1$, and remove every non-free edge in $P$ from $H_1$. Also add the free edge $(x,y)$ to $H_1$. Since these two types of edges form an alternating path, after we have done the mentioned `switching', each vertex in $X$ still has degree $d_1$ in $H_1$, while the degree of $t$ in $H_1$ increased by one. Furthermore, the only vertex in $Y$ which changed degree in $H_1$ is the vertex $y$, whose degree increased by one, and since $y\notin Y_{bad}$, each vertex in $Y$ still has degree at most $d_2$.

% \textbf{Removing an edge from $H_0$}. Suppose the adversary requests edge $(x,y)$ to be removed from $H_0$. If $x\in X$, then add the removed edge  $(x,y)$ to $H_1$, and note that now all invariants are satisfied again.

% If $x\notin X$, then by removing the edge $(x,y)$ from $H_0$, might cause that $d_H(y)<d_1/10$, so in that case we remove $y$ from $Y$. Now, we remove all vertices from $X$ which do not satisfy the second invariant, and all adjacent edges from $H_1$. Now, we again update $Y$, and continue this process until the first two invariants are both satisfied. 

% \textbf{Complexity.} When answering a request to add an edge to $H_0$, there are at most $n$ vertices to which we need to add at most $d$ edges in $H$; adding one of those edges is easily seen to be in $O(n)$. Hence, only $O(n^2d)$ steps are necessary to complete such a request. 
% On the other hand, when the request is to remove a vertex in $H_0$, it is easy to see that this can be done in $O(nd^2)$ time.

% \end{proof}
